LearnMate^2: Design and Evaluation of an LLM-powered Personalized and Adaptive Support System for Online Learning

Personalization is crucial for effective learning, yet online learning, designed for widespread availability and open access, lacks personalized guidance. Recent advancements in large language models (LLMs) offer opportunities to bridge this gap. We explore how LLM-driven tools may be designed to support personalized and adaptive learning and examine how they shape user experience and learning outcomes. We iteratively designed \tool{} to support online learning by providing personalized study plans, real-time contextual assistance, and adaptive learning activities. A preliminary study ($n=24$) assessed the effectiveness and usability of \tool{} and informed refinements in our system, which we then evaluated ($n = 16$) against a combination of a state-of-the-art online learning platform and an LLM for learning support. Results indicate that \tool{} advances AI pedagogy by improving both learning outcomes and user experience compared to existing online learning and support tools. This work advances our understanding of the design space of personalized, AI-driven educational tools and their potential impact on user experience.

==> figure_adapt.tex <==

\begin{figure*}[!tb]
  \includegraphics[width=\textwidth]{figures/Adapt.pdf}
  \Description[Adapting Task Results]{Five side-by-side bar charts comparing C1 (AdaptMate, pink) and C2 (Baseline, blue) on the adapting task (T3). Performance: AdaptMate approximately 5.6, Baseline approximately 4.8, significant difference (p < .05, marked *). Ease of Use: AdaptMate approximately 5.7, Baseline approximately 5.1, significant difference (p < .05, marked *). Ease of Learning: AdaptMate approximately 6.3, Baseline approximately 5.8, no significant difference. Satisfaction: AdaptMate approximately 5.3, Baseline approximately 4.4, significant difference (p < .05, marked *). SUS: AdaptMate approximately 77, Baseline approximately 71, no significant difference. Error bars indicate standard error.}
   \vspace{-12pt}
  \caption{\textit{Quantitative Data from User Study---} Bar graphs on participants' perceived performance of usefulness, ease of use, ease of learning, satisfaction and usability scores across different conditions for the adapting task (T3). Horizontal lines indicate significant pairwise comparisons with repeated measures ANOVA ($p < .05^{\ast}$, $p < .01^{\ast\ast}$, $p < .001^{\ast\ast\ast}$). Vertical lines in each bar graph indicate standard error. 
}
  \label{fig:adapt}
%   \vspace{-6pt}
\end{figure*}


% \begin{figure*}[!h]
%   \includegraphics[width=\textwidth]{figures/personalized plan.pdf}
%    \vspace{-12pt}
%   \caption{\textit{\ours{} Interface ---} The front-end interface for generating personalized learning plans. We outline the user's interaction with the front-end as a guide to explain the pipeline of \ours{} in Section \ref{sec:tec}.
  
% }
%   \label{fig:personalizedPlan}
% %   \vspace{-6pt}
% \end{figure*}





==> figure_adapt_system.tex <==

\begin{figure*}[!tb]
  \includegraphics[width=\textwidth]{figures/adapt_system.pdf}
  \Description[AdaptMate Interface]{A split-screen screenshot. The left panel shows a chat interface with three labeled regions. (k) A quiz question asking about evidence historians use to study Era 2, with four answer options (A–D) and clickable answer buttons. (l) A quiz performance analysis showing a score of 42.9\%, identifying three areas of confusion: differences between forager and farmer societies, nature of historical evidence in pre-literate eras, and specific details of key case studies. (m) An AdaptMate section titled "Now It's Adjustment Section" offering to generate a refined, performance-boosting plan. The right panel (n) shows an agenda-view calendar for September 10–October 10, 2025, listing adapted study sessions including targeted review sessions such as "Targeted Review: Food Surplus \& The Rise of Farming."}
   \vspace{-12pt}
  \caption{\textit{\texttt{AdaptMate} Interface ---} The front-end interface for adaptive plan refinement based on learning performance. After completing a study session and quiz, users receive a detailed performance report with learning insights (step \protect\darkgreysquare{l}). Users can then request plan adjustments (step \protect\darkgreysquare{m}), and \texttt{AdaptMate} generates an updated study plan that incorporates quiz results, interaction patterns, and prior preferences, presented in both text and calendar formats (step \protect\darkgreysquare{n}). We outline the user's interaction with the front-end as a guide to explain the pipeline of \texttt{AdaptMate} in Section \ref{sec:adaptmate}.
}
  \label{fig:adapt_system}
%   \vspace{-6pt}
\end{figure*}



==> figure_plan.tex <==

\begin{figure*}[!tb]
  \includegraphics[width=\textwidth]{figures/Plan.pdf}
  \Description[Planning Task Results]{Five side-by-side bar charts comparing C1 (PlanMate, pink) and C2 (Baseline, blue) on the planning task (T1) across five measures, all on a 1–7 scale except SUS which is 0–100. Performance: PlanMate approximately 5.5, Baseline approximately 4.5, no significant difference. Ease of Use: both approximately 5.5, no significant difference. Ease of Learning: both approximately 6, no significant difference. Satisfaction: PlanMate approximately 5.5, Baseline approximately 4, no significant difference. SUS: PlanMate approximately 75, Baseline approximately 65, no significant difference. Error bars indicate standard error.}
   \vspace{-12pt}
  \caption{\textit{Quantitative Data from User Study ---} Bar graphs on participants' perceived performance of usefulness, ease of use, ease of learning, satisfaction and usability scores across different conditions for the planning task (T1). Horizontal lines indicate significant pairwise comparisons with repeated measures ANOVA ($p < .05^{\ast}$, $p < .01^{\ast\ast}$, $p < .001^{\ast\ast\ast}$). Vertical lines in each bar graph indicate standard error. 
}
  \label{fig:plan}
%   \vspace{-6pt}
\end{figure*}


% \begin{figure*}[!h]
%   \includegraphics[width=\textwidth]{figures/personalized plan.pdf}
%    \vspace{-12pt}
%   \caption{\textit{\ours{} Interface ---} The front-end interface for generating personalized learning plans. We outline the user's interaction with the front-end as a guide to explain the pipeline of \ours{} in Section \ref{sec:tec}.
  
% }
%   \label{fig:personalizedPlan}
% %   \vspace{-6pt}
% \end{figure*}





==> figure_plan_system.tex <==

\begin{figure*}[!th]
  \includegraphics[width=\textwidth]{figures/plan_system.pdf}
  \Description[PlanMate Interface]{A screenshot of the PlanMate interface with five labeled regions. (a) A chat panel where a user types their learning goal in natural language, stating they want to self-study AP World History but feel overwhelmed by the curriculum. (b) A system guidance panel listing three steps: Click Plan to start planning, Click Study to start studying, and Click Adjust to refine the plan. (c) A chatbot response offering three preference buttons: Time, Pace, and Path. (d) A generated weekly study plan for "Week 1: Introduction to Big History" with a detailed daily schedule including specific topics and study tips. (e) An interactive calendar view showing September 2025 with color-coded study sessions populated across the month, including units, topics, and review sessions.}
   \vspace{-12pt}
  \caption{\textit{\texttt{PlanMate} Interface ---} The front-end interface for personalized study planning. Users begin by specifying their learning goals in natural language (step \protect\darkgreysquare{a}), then provide preferences across multiple dimensions, including time availability, learning pace, and content path (steps \protect\darkgreysquare{b} to \protect\darkgreysquare{c}). Based on these inputs, \texttt{PlanMate} generates a personalized study plan in text form (step \protect\darkgreysquare{d}) and visualizes it as an interactive calendar schedule (step \protect\darkgreysquare{e}).We outline the user's interaction with the front-end as a guide to explain the pipeline of \texttt{PlanMate} in Section \ref{sec:planmate}.
}
  \label{fig:plan_system}
%   \vspace{-6pt}
\end{figure*}

% \caption{\textit{\ours{} Interface ---} The front-end interface for course selection. Users begin by defining their learning \textit{goals} through either: (1) specifying learning interests (step \protect\darkgreysquare{a}) to generate course recommendations (step \protect\darkgreysquare{b}), or (2) browsing courses by topic (step \protect\darkgreysquare{c}). We outline the user’s interaction with this interface as a guide to explain the pipeline of \ours{} in Section \ref{goalGuidelines}.
  
% \begin{figure*}[!h]
%   \includegraphics[width=\textwidth]{figures/personalized plan.pdf}
%    \vspace{-12pt}
%   \caption{\textit{\ours{} Interface ---} The front-end interface for generating personalized learning plans. We outline the user's interaction with the front-end as a guide to explain the pipeline of \ours{} in Section \ref{sec:tec}.
  
% }
%   \label{fig:personalizedPlan}
% %   \vspace{-6pt}
% \end{figure*}





==> figure_quiz_new.tex <==

\begin{figure}[!tb]
  \includegraphics[width=\columnwidth]{figures/Quiz_new.pdf}
  \Description[Quiz Results]{Two side-by-side bar charts comparing quiz scores between C1 (LearnMate², shown in pink) and C2 (Baseline, shown in blue). Quiz 1 (out of 15): LearnMate² scored approximately 13, Baseline approximately 11, with a statistically significant difference (p < .05, marked with *). Quiz 2 (out of 10): LearnMate² scored approximately 7.9, Baseline approximately 6, with a statistically significant difference (p < .01, marked with **). Error bars indicate standard error.}
   \vspace{-12pt}
  \caption{\textit{Quantitative Data from User Study---}
  Bar graphs show participants' quiz results for Quiz 1 and Quiz 2. Horizontal lines indicate significant pairwise comparisons with paired t-tests ($p < .05^{\ast}$, $p < .01^{\ast\ast}$, $p < .001^{\ast\ast\ast}$). Vertical lines in each bar graph indicate standard error.
}
  \label{fig:quiznew}
%   \vspace{-6pt}
\end{figure}


% \begin{figure*}[!h]
%   \includegraphics[width=\textwidth]{figures/personalized plan.pdf}
%    \vspace{-12pt}
%   \caption{\textit{\ours{} Interface ---} The front-end interface for generating personalized learning plans. We outline the user's interaction with the front-end as a guide to explain the pipeline of \ours{} in Section \ref{sec:tec}.
  
% }
%   \label{fig:personalizedPlan}
% %   \vspace{-6pt}
% \end{figure*}





==> figure_quiz_old.tex <==

\begin{figure*}[!tb]
  \includegraphics[width=0.7\textwidth]{figures/Quiz_old.pdf}
   \vspace{-12pt}
  \caption{\textit{Quantitative Data from Preliminary User Studies ---}
  Bar graphs show participants' quiz results for Quiz 1 (\textit{2.1 Era 2 Overview}) and Quiz 2 (\textit{3.1 Era 3 Overview}). 
  Horizontal lines indicate significant pairwise comparisons with paired t-tests ($p < .05^{\ast}$, $p < .01^{\ast\ast}$, $p < .001^{\ast\ast\ast}$). Vertical lines in each bar graph indicate standard error.
}
  \label{fig:quizold}
%   \vspace{-6pt}
\end{figure*}



==> figure_scale.tex <==

\begin{figure*}[!th]
  \includegraphics[width=\textwidth]{figures/Scale.pdf}
   \vspace{-12pt}
  \caption{\textit{\ours{} USE and SUS data} no description.}
  \label{fig:scale}
\end{figure*}

% \begin{figure*}[!th]
%   \includegraphics[width=\textwidth]{figures/course_select.pdf}
%    \vspace{-12pt}
%   \caption{The \ours{} \textit{course selection} interface. Users begin by defining their learning \textit{goals} through either: (1) specifying learning interests (step \protect\darkgreysquare{a}) to generate course recommendations (step \protect\darkgreysquare{b}), or (2) browsing courses by topic (step \protect\darkgreysquare{c}). We outline the user’s interaction with this interface as a guide to explain the pipeline of \ours{} in Section \ref{goalGuidelines}.
% }
%   \label{fig:courseSelection}
% %   \vspace{-6pt}
% \end{figure*}


% \begin{figure*}[!th]
%   \includegraphics[width=\textwidth]{figures/Interface.pdf}
%    \vspace{-12pt}
  
%   \caption{\textit{\ours{} Interface ---} 
%  The front-end interface of \ours{}. We outline the user's interaction with the front-end as a guide to explain the pipeline of \ours{} in Section \ref{sec:tech}.}
  

%   \label{fig:interface}
% %   \vspace{-6pt}
% \end{figure*}





==> figure_study.tex <==

\begin{figure*}[!b]
  \includegraphics[width=\textwidth]{figures/Study.pdf}
\Description[Studying Task Results]{Five side-by-side bar charts comparing C1 (StudyMate, pink) and C2 (Baseline, blue) on the studying task (T2). Performance: StudyMate approximately 5.9, Baseline approximately 4.1, significant difference (p < .001, marked ***). Ease of Use: StudyMate approximately 5.7, Baseline approximately 4.9, significant difference (p < .05, marked *). Ease of Learning: StudyMate approximately 6.3, Baseline approximately 5.6, no significant difference. Satisfaction: StudyMate approximately 5.5, Baseline approximately 4.0, significant difference (p < .001, marked ***). SUS: StudyMate approximately 76, Baseline approximately 65, significant difference (p < .05, marked *). Error bars indicate standard error.}
   \vspace{-12pt}
    \caption{\textit{Quantitative Data from User Study---} Bar graphs on participants' perceived performance of usefulness, ease of use, ease of learning, satisfaction and usability scores across different conditions for the studying task (T2). Horizontal lines indicate significant pairwise comparisons with repeated measures ANOVA ($p < .05^{\ast}$, $p < .01^{\ast\ast}$, $p < .001^{\ast\ast\ast}$). Vertical lines in each bar graph indicate standard error. 
}
  \label{fig:study}
%   \vspace{-6pt}
\end{figure*}


% \begin{figure*}[!h]
%   \includegraphics[width=\textwidth]{figures/personalized plan.pdf}
%    \vspace{-12pt}
%   \caption{\textit{\ours{} Interface ---} The front-end interface for generating personalized learning plans. We outline the user's interaction with the front-end as a guide to explain the pipeline of \ours{} in Section \ref{sec:tec}.
  
% }
%   \label{fig:personalizedPlan}
% %   \vspace{-6pt}
% \end{figure*}





==> figure_study_system.tex <==

\begin{figure*}[!th]
  \includegraphics[width=\textwidth]{figures/study_system.pdf}
  \Description[StudyMate Interface]{A split-screen screenshot. The left panel shows a chat interface. (f) The chatbot prompts the user to select a unit to begin, offering "2.1 Cities, Societies, and Empires" and "3.1 Cities, Societies, and Empires," and displays a 30-minute study plan. (g) The study session starts with buttons for "Ask a Question" and "End Study." (h) A user asks "How did the New Stone Age society form?" (i) The chatbot responds with a contextually grounded answer citing course content at timestamp 4:35, explaining the Neolithic transition, with expandable options for More Details, External Resources, and Practice Questions. The right panel (j) shows a YouTube video player displaying a Khan Academy World History Project video "WHP Origins | Era 2 Overview" paused at 4:33, with an illustration of early human figures.}
   \vspace{-12pt}
  \caption{\textit{\texttt{StudyMate} Interface ---} The front-end interface for interactive learning support during scheduled study sessions. Users start a learning session by selecting a planned time slot (step \protect\darkgreysquare{f}), after which \texttt{StudyMate} provides session-specific guidance. During the session, users can ask questions and receive contextual assistance with progressive disclosure options, including more details, practice questions, and external resources (steps \protect\darkgreysquare{g} to \protect\darkgreysquare{i}). At the end of the session, \texttt{StudyMate} generates an adaptive quiz to assess learning outcomes (step \protect\darkgreysquare{k}). We outline the user's interaction with the front-end as a guide to explain the pipeline of \texttt{StudyMate} in Section \ref{studymate}.
  \textit{Screenshot © Khan Academy (khanacademy.org), used under CC BY-NC-SA 4.0.}
}
  \label{fig:study_system}
%   \vspace{-6pt}
\end{figure*}


% \begin{figure*}[!h]
%   \includegraphics[width=\textwidth]{figures/personalized plan.pdf}
%    \vspace{-12pt}
%   \caption{\textit{\ours{} Interface ---} The front-end interface for generating personalized learning plans. We outline the user's interaction with the front-end as a guide to explain the pipeline of \ours{} in Section \ref{sec:tec}.
  
% }
%   \label{fig:personalizedPlan}
% %   \vspace{-6pt}
% \end{figure*}





==> figure_system.tex <==
\begin{figure*}[!tb]
  \includegraphics[width=\textwidth]{figures/System_workflow.pdf}
   \vspace{-12pt}
  \caption{\textit{\ours{} System Workflow ---} 
  The front-end interface of \tool{} (left) and the system workflow (right). The three-step integrated learning loop shows how \texttt{PlanMate}, \texttt{StudyMate}, and \texttt{AdaptMate} work together to provide personalized study planning, real-time contextual assistance, and adaptive learning activities that adjust based on user progress and performance.
  We outline and explain the pipeline of \tool{} in Section~\ref{sec:system}.
  \textit{Screenshot © Khan Academy (khanacademy.org), used under CC BY-NC-SA 4.0.}}
  \label{fig:system_workflow}
  \Description[LearnMate² System Workflow]{A diagram showing the LearnMate² front-end interface on the left and the system pipeline on the right. The pipeline is divided into three steps. Step 1, PlanMate, shows the system providing personalized study plan guidance, configuring learning preferences based on user input, and generating a personalized study plan displayed in a calendar. Step 2, StudyMate, shows the user beginning a study session, receiving session-specific guidance, getting real-time contextual assistance, completing learning, and taking an adaptive quiz. Step 3, AdaptMate, shows the system generating a quiz report and adapting the study plan based on performance, experience, and preferences.}
\end{figure*}


==> figure_teaser.tex <==
\begin{teaserfigure}
  \includegraphics[width=0.85\textwidth]{figures/teaser.pdf}
   \vspace{-12pt}
  \caption{\textit{\ours{} --- } In this work, we present \ours{}, a system designed to improve online learning through three main components. The figure contrasts the current online learning workflow (left), where students face challenges such as cold start problems (depicted as step \protect\darkgreysquare{A}), lack of timely and effective help (step \protect\darkgreysquare{B}), and fixed learning plans (step \protect\darkgreysquare{C}), with the \ours{} workflow (right). 
  To address these challenges, \ours{} integrates \texttt{PlanMate}, which offers structured guidance to help learners get started and generate personalized study plans based on goals, time, path, and pace (step \protect\darkgreysquare{A}); \texttt{StudyMate}, which provides real-time contextual assistance with progressive disclosure (step \protect\darkgreysquare{B}); and \texttt{AdaptMate}, which adjusts learning activities dynamically based on quiz performance and progress (step \protect\darkgreysquare{C}). 
  Together, these components enable a personalized, adaptive, and supportive online learning experience.
}
  \label{fig:system_workflow}
%   \vspace{-6pt}
\end{teaserfigure}

% \caption{\textit{\ours{} --- }In this work, we present \ours{}, a system that applies formal verification techniques to LLM outputs for end-user planning tasks. The figure compares a user's interaction with an LLM without \ours{} (left) and with \ours{} (right). In both cases, the user provides a prompt requesting a plan with specific requirements (depicted as step \protect\darkgreysquare{A}). The LLM generates an initial planning attempt from the prompt (step \protect\darkgreysquare{B}). With \ours{}, however, rules are automatically extracted from the user's prompt, verified, and refined through direct user involvement (step \protect\darkgreysquare{C}). These rules are then sent to the model checker, which verifies whether the LLM's output adheres to the user-defined rules (step \protect\darkgreysquare{D}). The validation result, along with any rule violations, is shared with both the user and the LLM to refine future planning outputs (step \protect\darkgreysquare{E}). 

==> related_llm.tex <==

% \subsection{personalization/adaptation efforts in ml}


\subsection{Personalization and Adaptation in the Era of LLMs}

In the era dominated by LLMs, encompassing commercial LLMs (\eg GPT-4~\cite{gpt-4}, Gemini families~\cite{geminiteam2023gemini}, and Claude~\cite{claude}) and ``open source'' LLMs (\eg LLaMA~\cite{touvron2023llama}, Grok~\cite{grok}, and Mistral~\cite{jiang2023mistral}), we have witnessed the remarkable capabilities of these models in generating human-like text and understanding contextual cues.
Nonetheless, just having an LLM generate answers based on its pre-training has a clear limitation: although the most-capable LLMs have been trained on large swaths of the internet, they would not have seen documents generated past a specific training cutoff date, and certainly could not have seen personal/enterprise documents, documents behind paywalls, data in databases, and so on.
To overcome such limitation, there are two common approaches for incorporating domain-specific information into LLMs for their personalized usage: fine-tuning and Retrieval Augmented Generation (RAG).
% has fostered a new level of personalization and adaptation.

% LLMs have been extensively used for personalization, thanks to their ability to model user interactions and generate responses that align with user's needs and preferences. 
% For instance, GPT-2 was used by~\citet{radford2019language} to generate personalized responses in dialogue systems, thereby enhancing user engagement. Similarly,~\citet{zhang2020dialogpt} employed BERT for personalizing chatbots, making responses more contextually relevant and personalized, and consequently improving user experience.

% Personalization and adaptation using LLMs have commonly relied on two key approaches: fine-tuning and Reinforcement Learning from Human Feedback (RLHF). 
Fine-tuning involves adapting the pre-trained LLM to a specific task or user data by continuing the training process, thereby enabling the models to learn the nuances and requirements of the target domain~\cite{houlsby2019parameter, zhang2020dialogpt}. 
However, the fine-tuning approach requires substantial computational resources and expertise, as well as full white-box access to the model's internals, which is not a realistic assumption since LLM model weights are often protected by the model provider's intellectual property laws.
Moreover, it risks catastrophic forgetting, where the model loses its ability to perform tasks it was previously good at, and the severity of forgetting increases as the model scale increases~\cite{luo2023empirical}. 
Other than adaptation to target task, Reinforcement Learning from Human Feedback (RLHF) can help align LLMs with user preferences~\cite{bai2022rlhf}.
RLHF involves the additional steps of training a Reward Model with preference data, which consists of prompts and multiple candidate outputs ranked by human evaluators. Then it uses the reward model to fine-tune the LLM through reinforcement learning 
to align the LLM's behavior with human preferences and values defined via reward modeling.
% This approach, used by Bahdanau et al., (2018) for training a dialogue system, allows for continuous model improvement. 
% Bahdanau, D., Chattopadhyay, A., Serdyuk, D., Wallach, H., & Courville, A. (2018). An actor-critic algorithm for sequence prediction. In International Conference on Learning Representations (ICLR).
Yet, the performance of RLHF largely depends on reward modeling and the quality and quantity of human feedback, which can be challenging to obtain, and it shares the computational expense and complexity of the fine-tuning approach. This makes fine-tuning and RLHF-based approaches less accessible to individual users who may want to leverage state-of-the-art off-the-shelf LLMs like GPT-4, OpenAI's Codex, or Google's LaMDA for personal use.

% A more recent alternative to these methods is the Retrieval-Augmented Generation (RAG) approach. Just having an LLM generate answers based on its pre-taining has two limitations: (a) although the most-capable LLMs have been trained on large swaths of the internet, they would not have \textit{seen} documents generated past a specific training cutoff date, and certainly could not have seen personal/enterprise documents, documents behind paywalls, data in databases, and so on. (b) Even if an LLM generates an answer, there is no way to verify the validity of the answer as it does not include a source citation. 
On the other hand, RAG provides more flexibility to adapt to changing data without retraining the entire model, by only requiring black-box access to the model (\ie via API calls).
It allows the model to leverage knowledge sources (\eg specific documents on personal information or instructions, or an external database) not present in the original training data of the deployed LLM. 
It retrieves relevant information from the external knowledge and uses it to guide the response generation by augmenting the user input prompt~\cite{lewis2020retrieval}.  
% The RAG approach addresses both of these limitations by retrieving relevant information from a knowledge source (\eg specific documents or an external database) and using it to guide the response generation~\cite{lewis2020retrieval}.
% RAG combines the strengths of powerful pre-trained models and information retrieval to generate responses~\cite{lewis2020retrieval}. 
% This method is computationally efficient and versatile, and more importantly,
% RAG can be used with just API access to the LLMs, making it a more accessible approach for individuals wanting to make adaptive use of any black-box LLMs for personal use cases.
This method is not only computationally efficient and versatile, compared to fine-tuning or RLHF approaches that necessitate additional training, but is also accessible to individuals who wish to adaptively use any black-box LLMs for personal use cases.
% , as it only requires API access to the LLMs.
More importantly, it is possible with RAG to verify the validity of the generated answer by including a source citation. 


There have been a few recent attempts to explore the use of RAG in the context of personalized dialogue generation, such as persona profiles and distinctive authorial nuances~\cite{rag-style, lapdog}. 
% \citet{rag-style} proposes a style-based RAG approach, where the style embeddings are used to capture distinctive authorial nuances for the purpose of personalizing LLMs. 
However, the focus of personalization in our work rather lies in handling conflicting multiple user requests and supporting decision-making adapted to individual preferences and instructions.
To the best of our knowledge, our work is the first to propose a RAG approach with usability for multi-user adaptive personalization.
Moreover, we explore the potential of multi-agent collaboration to address complex personalization requests, in contrast to the monolithic agent-based approaches found in most prior works on RAG-based personalization.
% In conclusion, the era of LLMs has brought significant advancements and opportunities in personalization and adaptation. Despite the challenges, with the right strategies and methodologies such as RAG, these models can offer rich, engaging, and personalized user experiences.

